Certified Graph View Maintenance with Regular Datalog

We employ the Coq proof assistant to develop a mechanically-certified framework for evaluating graph queries and incrementally maintaining materialized graph instances, also called views. The language we use for defining queries and views is Regular Datalog (RD) -- a notable fragment of non-recursive Datalog that can express complex navigational queries, with transitive closure as native operator. We first design and encode the theory of RD and then mechanize a RD-specific evaluation algorithm capable of fine-grained, incremental graph view computation, which we prove sound with respect to the declarative RD semantics. By using the Coq extraction mechanism, we test an Ocaml version of the verified engine on a set of preliminary benchmarks. Our development is particularly focused on leveraging existing verification and notational techniques to: a) define mechanized properties that can be easily understood by logicians and database researchers and b) attain formal verification with limited effort. Our work is the first step towards a unified, machine-verified, formal framework for dynamic graph query languages and their evaluation engines. This paper is under consideration for acceptance in TPLP.

==> appref.tex <==
\bibliographystyleC{acmtrans}
{\small\bibliographyC{paper-bib}}


==> coqcomment.tex <==
In order to construct the formal specification of our graph database model, of its query language and of its IVMGD evaluation engine, we follow a methodology based 
on \emph{theorem proving} techniques. These are aimed at building and at verifying theorems using software, whose trusted kernel is based on a 
specific set of inference rules. This concept can be traced back to the Automath project \citeC{Bruijn} and 
to Milner's \emph{Logic of Computable Functions} (\textsc{LCF}) architecture \citeC{Milner}, whose kernel implements natural deduction. 
Theorem provers can either discharge obligations \emph{automatically} or \emph{interactively}, by requiring users to work in tandem with the computer.
Throughout this paper, we relied on the latter approach. In this setting, a typical workflow consists of providing an input program, together with its specification,
and helping the prover construct a (mechanized) proof that the program's output complies with the specification.
Consequently, the problem of ensuring program soundness is reduced to that of ensuring the soundness of the underlying specification. To this end, we 
employed the \coq proof assistent and its \textsc{ssreflect} extension. 

\subsection{\textsc{Coq}}\label{sec:coq}

The \textsc{Coq} proof assistant belongs to the class of interactive theorem provers, alongside systems from the \textsc{HOL} family, e.g., 
\textsc{Isabelle/HOL} (\citeC{Nipkow}), \textsc{HOL-light} (\citeC{Harrison}), \textsc{PVS} (\citeC{Owre}), -- in the classic higher-order logic tradition --
and alongside systems such as \textsc{NuPrl} (\citeC{Constable}), \textsc{Agda} (\citeC{Norell}) and \textsc{Matita} (\citeC{Asperti}) -- in the constructive type theory 
tradition. Its core formalism is the Calculus of Inductive Constructions (\textsc{CIC}) \citeC{Paulin}, which corresponds to the most expressive type theory in Barendregt's 
lambda cube \citeC{Barendregt}, namely that supporting polymorphism, type operators and dependent types. The \textsc{Coq} system and its underlying theory are described in 
\citeC{Bertot}.

The Calculus of Inductive Constructions is based on the Curry-Howard ``propositions-as-types and proofs-as-programs''
paradigm (\citeC{Curry}, \citeC{Howard}). As such, \textsc{Coq} is both a proof system and a functional programming language (Gallina). Essentially, the 
type system can be seen as containing only function types and inductive types. \textsc{Coq}'s equality is \textit{intensional}
and type checking is decidable. The system in implemented in Objective Caml, a dialect of \textsc{ML}, 
and comes with an automatic extraction mechanism from \textsc{Coq} proof specifications that 
can be used to build certified and efficient functional programs. Proving a theorem $T$ in \textsc{Coq} involves
finding a program $p$, such that $\vdash p : T$, i.e, that $p$ inhabits the type $T$. Alternatively, it involves constructing
a typing derivation that assigns the type $T$ to the program $p$. 

A classical example of a proposition is the ``and'' datatype with a single constructor, encapsulating two proofs, 
usually written as \C|/\|. To prove $A \wedge B$, one needs to find a proof $a$ for $A$ and a proof $b$ for $B$ and 
then apply the conjunction constructor. A more interesting datatype is \C|\/|. This datatype has two constructors,
indicating whether one has found a proof either for $A$ or for $B$. It is easy to see that to provide a proof for
the excluded middle principle, i.e, $A \vee \neg A$, one would have to find a proof for either $A$ or $\neg A$. 
This is unprovable in general, as there exist propositions that cannot be decided in this way.
For example, if $A$ expresses Turning machine termination, the principle is equivalent to the halting problem.
Similarly, to prove $\exists x, P x$, one has to provide a witness $w$ and a proof of $P w$. Consequently,
$\neg (\forall x, \neg P x)$ does not imply $\exists x, P x$, as this is equivalent to the excluded middle.

As building programs by hand is cumbersome, \textsc{Coq} provides a set of so called \emph{tacticals}, for building
Gallina programs. We will discuss tacticals more in the following section.

\subsection{\textsc{SSReflect}}\label{sec:coq}

We base our work on the \textsc{Mathematical Components} library\footnote{\url{http://math-comp.github.io/math-comp/}}, built using the \textsc{Ssreflect} (\citeC{GonthierSR}) extension of \textsc{Coq}. This library is especially well-suited for our purposes, as it
was the basis of extensive formalizations of finite model theory, in the context of proving the Feit-Thompson theorem (\citeC{GonthierFT}), central to finite group classification.

\paragraph{Tactics}  

A comprehensive presentation of \textsc{Ssreflect} functionalities is in \cite{GonthierSR}. In the following, ee briefly overview the most important tactics.
Generally, the tactics \textsc{Ssrflect} provides can be split in two types: the ``defective'' tactics, i.e, \C|move|, \C|case|, \C|have|, \C|elim| and \C|apply|, 
which behave similarly to their \textsc{Coq} counterparts, and the rewrite tractics, comprising unfolding, simplification and rewrite. Tactics are additionally constructed combining the
``defective'' ones with context-manipulation ``tacticals'', i.e, \C|:| and \C|=>|. The former moves facts and constants to the goal, while the latter introduces variables, 
local definitions and assumptions to the context. \textsc{ssreflect} supports pattern selection mechanisms common to all tactics. \\

The defective \C|move| tactic exposes the first assumption in goals, i.e, changing \C|$\sim$ P| to \C|P $\rightarrow$ False|. The defective \C|case| tactic does case analysis 
on (co)inductive types, by deconstructing them, exposing their constructors and arguments and instantiating the latter correspondingly; it also does injection, if it finds an equality. 
The defective \C|elim| tactic performs inductive elimination on inductive types. Finally, backwards chaining reasoning is implemented via \C|apply|. A convenient feature is that these tactics can be chained with
views, allowing to change boolean equality goals into equivalent propositions.

\paragraph{Library Overview}

The \textsc{Mathematical Components} library provides a development ranging from basic data structures and types
to linear algebra, Galois and finite group theory. In particular, the support for finite types is mature,
as it lies at the basis of many other developments. The library is organized in an object-oriented way, 
with types implementing interfaces and mixins implementing interface inheritance. 
The low level implementation of the class system is done by the canonical structures mechanism, allowing users to
supply solutions to particular unification problems involving records; this is detailed in \citeC{MathStruct}.
Next, we quickly present the main classes and libraries we used.

\begin{description}
 \item[ssrfun] The file contains the main lemmas and definitions about functions. 
 For instance, lemmas about injectivity.
 \item[ssrbool]The \textsc{Mathematical Components} library is highly specialized in dealing with \emph{decidable predicates}. This file
  develops their corresponding base theory.\\ Decidable predicates are predicates whose truth can be computationally determined or, 
  in \textsc{Coq} terms, \C|P : Prop|, such that \C|{P} + {not P}| is 
  provable~\footnote{The ``+'' operator is the computational version of ``or''. }.  It is often convenient to
  represent the truth of \C|P| as a concrete algorithm \C|p : bool|.\\ Indeed, \C|reflect P p|
  does exactly that, i.e, \C|reflect P true| is provable only when \C|P| is provable and \C|reflect P false| is provable only
  when \C|not P| is provable. \\The \C|ssrbool| file also provides support for 
 \emph{generic predicates}, e.g, the \verb!\in! predicate, widely used in the library to implement membership 
 comprehensively, allowing one to, for instance, write 
 \verb!x \in l = x \in s!, where \C|l| is a list and \C|s| is a set. 
 \item[eqtype] The file provides the base class of the \textsc{Mathematical Components} hierarchy: the \C|eqType| class of types 
 with decidable equality, written \verb!x == y!. The main corresponding lemma is \C|eqP|, 
 which states that the computational equality corresponds to the propositional one, i.e \verb!(x = y) <-> (x == y)!.
 Also, this file contains the \C|subType| class, which provides generic support for well-behaved sigma types of the form 
 \C|{x $\mid$ P x}|, where \C|P| is a boolean predicate. A subtype coerces to the base type automatically, and thanks to 
 the boolean nature of \C|P|, the proof is irrelevant, allowing us to transfer all the properties of the base type 
 to the subtype.
 \item[ssrnat] The file provides a theory of the natural numbers, with the more covenient choice of boolean operators 
 for orders, e.g, given two natural numbers \C|m| and \C|n|, the less or equal comparison \C|leq| is defined as computationally
 checking \verb!m - n == 0!.
 \item[seq] The file provides a theory of lists or sequences, with generic predicate membership, i.e, \verb!(x \in l)!, 
 if \C|x| is an \C|eqType|. 
 \item[fintype] The file is crucial to our development, as it provides the \C|finType| class of finite types.
 Finiteness is defined as the duplicate-free enumeration of elements of a given type, i.e,
 \C|forall x : T, count x (enum T) = 1|. The library also provides the type of ordinals
 \C|'I_n = { m : nat $\mid$ m < n }|. Moreover, we take advantage of the finType instance for tuples, 
 which provides a convenient way of encoding, for example, a program's Herbrand base, given the maximal arity 
 \C|n| of its predicates and  its active domain \C|adom|, i.e, \C|enum (n.-tuple adom)|. 
 Another interesting property supported by the library
 is that quantification becomes decidable. For this purpose, the following constructs are supported:
 \C|[forall x, P x]| and \C|[exists x, P x]|, together with the reflection lemmas \C|forallP|
 and \C|existsP|, relating the computational definitions of quantification to their usual counterparts. 
 This is very handy, as, in this setting, classical logic principles hold, e.g, 
 \C|$\sim$ $\sim$[forall x , $\sim$ $\sim$ P x] = [exists x, P x]|.
 \item[finfun] The file provides a theory of finitely-supported functions. Given a finite type,
 functions from it are represented extensionally as their graph, i.e the list of values the function
 assigns to every domain element. 
 \item[finset] The file provides a theory of sets over finite types. Given an underlying finite type, 
 these are represented as a lists of booleans, corresponding to the set membership or characteristic
 function. The main property is set extensionality (\C|setP|), i.e, \verb!(forall x, x \in s1 = x \in s2) <-> s1 = s2!, 
 which is very convenient property for reasoning about sets point-wise.
 \item[bigop] We also take advantage of the big operator library (see \citep{Bertot}), which adds monoid
 classes to the Mathematical Components hierarchy. This library provides us with indexed operators of the 
 form:
 \begin{center}
 \C|\bigop[op/zero]_l (fun x => P x)|.
 \end{center}
 In particular, by instantiating the operator \C|op| and the lower limit \C|zero| 
 with \C|setU| and, respectively, \C|set0|, we obtain set union and, by instantiating them with \C|addn| and \C|0|, we obtain
 the big sum. 
\end{description}


==> gupta-alg.tex <==

\begin{algorithm}[h!]
 \caption{Delta-Join Incremental View Maintenance}\label{euclid}
 {\hspace*{\algorithmicindent} 
 \textbf{Input} \small{   
   \[ 
   \begin{array}{lll}
   \Pi_{\mathcal{G}} & = & \text{RQ program}\\
   \mathcal{V}[\mathcal{G}] & = & \text{view materializations (stored evaluations of $\mathcal{V}_{\Pi}$, i.e., of the derived relations in $\Pi_{\mathcal{G}}$)}  \\
   \Delta \mathcal{G} & = & \text{graph updates (updates of $\mathcal{G}_{\Pi}$, i.e., of the base relations in $\Pi_{\mathcal{G}}$)} \\
   \end{array}
  \]}
   \hspace*{\algorithmicindent} 
  \textbf{Output} \small{  
   \[ 
   \begin{array}{lll}
   \Delta \mathcal{V} [\mathcal{G}; \Delta \mathcal{G}] & = & \text{incremental view updates (updates of $\mathcal{V}_{\Pi}$)} \\
   \end{array}
  \]}}
    \begin{algorithmic}[1]
    \Procedure{DeltaJoin}{}
     \For{$V \in \mathcal{V}_{\Pi} $}
     \State $V^{\nu} \gets V[\mathcal{G}] $
     \State $\Delta V \gets \emptyset$
     \EndFor
     \For{$i=n$ to $1$} 
     \For{$C_i \in \Pi_{\mathcal{G}}$} \Comment{Bottom-Up Processing}
     \State $\Delta V_i[\mathcal{G}; \Delta \mathcal{G}] \gets \delta(V_{i}) $
     \State $\Delta \mathcal{G} \gets \Delta \mathcal{G} \cup \Delta V_i[\mathcal{G}; \Delta \mathcal{G}]$
     \State $V_{i}^{\nu} \gets V \cup \Delta V_i[\mathcal{G}; \Delta \mathcal{G}] $
     \EndFor
     \EndFor
     \State $\Delta \Omega[\mathcal{G}; \Delta \mathcal{G}] \gets \delta(\Omega)$
     \State $\Omega[\mathcal{G}; \Delta \mathcal{G}] \gets \Omega[\mathcal{G}] \cup \Delta \Omega[\mathcal{G}; \Delta \mathcal{G}]  $
     \State \Return $\Omega[\mathcal{G}; \Delta \mathcal{G}]$
%   \State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
%    \State \textbf{goto} \emph{top}.
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> header.tex <==
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage{comment}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{mathabx}
%\usepackage{colonequals}
\usepackage{tikz}
%\usepackage{subfigure}
\usepackage{verbatim}
\usepackage{float}
%\usepackage{xspace}
%\usepackage{url}
%\usepackage{ifthen}
%\usepackage{stmaryrd}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{float}
%\usepackage{multirow,hhline}
%\usepackage{amsfonts,mathrsfs}
%\usepackage{stmaryrd}


% for the letter to the reviewers
\newcommand{\rrc}{\color{blue}}

\setlength{\marginparwidth}{3cm}

% \newcommand{\rmargin}[1]{%
% 
%   \marginpar{%
%     \rrc%
%     \raggedright%
%     \fontsize{8.5}{8.5}%
%     \selectfont%
% 
% \ifthenelse{\isodd{\thepage}}
%    {
% \begin{tabular}{cc}
% \begin{minipage}{2.5cm}#1\end{minipage}
% \end{tabular}
% 	}
%   {#1}
%   }
% }
% 
% 
% \newcommand{\rbox}[1]{{%
%     \begin{center}%
%     \rrc%
%     \frame{%
%       \frame{%
%         \parbox{\textwidth}{%
%           \smallskip
%           #1%
%           \smallskip
%         }%
%       }%
%     }%
%     \end{center}%
% }}
% 


%\newcommand{\rmark}{\marginpar{\rrc$\bigstar$}}
\newcommand{\rnew}[1]{{\rrc #1}}

\newcommand{\rone}{\textsc R_1}
\newcommand{\rtwo}{\textsc R_2}

%\newcommand{\COMMENT}[1]{\qquad\\\fcolorbox{red}{white}{\parbox{13cm}{#1}}}

\newcommand{\COMMENTT}[1]{\color{red!50}\noindent\rule{14cm}{0.1pt}\newline\color{black}#1\color{red}\newline\noindent\rule{14cm}{0.6pt}\color{black}\newline}



\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1.5pt] (char) {#1};}}




% for the paper

\usetikzlibrary{patterns,shapes,snakes}

\newcommand{\sig}{\mathit{sig}}
\newcommand{\insig}{\mathit{inSig}}
\newcommand{\outsig}{\mathit{outSig}}

\newcommand{\learner}{\mathit{learner}}
\newcommand{\CS}{\mathit{CS}}
\newcommand{\cs}{\mathit{CS}}
\renewcommand{\k}{\P(\P(\Omega_{\Rin}))^{\leq k}}
\newcommand{\C}{\mathcal{C}}
\renewcommand{\S}{\mathscr{S}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\N}{\mathbb{N}}
%\renewcommand{\P}{\mathcal{P}}
\newcommand{\Rin}{\mathcal{R}_\mathit{in}}
\newcommand{\Rout}{\mathcal{R}_\mathit{o}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\from}[2]{{\bf [{\sc \textcolor{red}{from #1: #2}}]}}
\newcommand{\attrs}{\mathit{attrs}}
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}
\newcommand{\Cert}{\mathit{Cert}}
\newcommand{\minus}{\mathop{\setminus}}
\newcommand{\Uninf}{\mathit{Uninf}}
\newcommand{\opt}{\mathrm{OPT}}
\newcommand{\sat}{\mathit{3SAT}}
\newcommand{\nn}{\mathit{NN}}
\newcommand{\RND}{\mathrm{RND}}
\newcommand{\BU}{\mathrm{BU}}
\newcommand{\TD}{\mathrm{TD}}
\newcommand{\Ls}{\mathrm{L^1S}}
\newcommand{\Lss}{\mathrm{L^2S}}
\newcommand{\Lsss}{\mathrm{L^kS}}
\newcommand{\bis}{\mathit{best\_in\_skyline}}
\newcommand{\skyline}{\mathit{skyline}}
\newcommand{\entropy}{\mathit{entropy}}
\newcommand{\twoentropy}{\mathit{entropy}^2}
\newcommand{\cons}{\mathrm{CONS}}
\newcommand{\minpos}{\mathrm{MIN\_POS}}
\newcommand{\uni}{\mathrm{UNINF}}

\renewcommand{\j}{\textit{Join}}
\newcommand{\uj}{\textit{UJoin}}
\renewcommand{\dj}{\textit{Join}^\ltimes}
\newcommand{\duj}{\textit{UJoin}^\ltimes}

\newcommand{\K}{\mathsf{K}}
\newcommand{\jc}{\mathsf{Join}}
\newcommand{\ujc}{\mathsf{UJoin}}
\newcommand{\djc}{\mathsf{Join}^\ltimes}
\newcommand{\dujc}{\mathsf{UJoin}^\ltimes}

%%% ALGORITHMS %%%
\floatstyle{ruled}
\newfloat{float@algorithm}{htbp}{loa}
\floatname{float@algorithm}{Algorithm}
\newcounter{LineCounter@algorithm} % line number counter

\newenvironment{BasicCommands@algorithm}{%
  \newcommand{\TAB}{\makebox[4ex][r]{}}%
  \newcommand{\ALGORITHM}{\textbf{algorithm}\xspace}%
  \newcommand{\INPUT}{\textbf{Input}\xspace}%
  \newcommand{\OUTPUT}{\textbf{Output}\xspace}%
  \newcommand{\ERROR}{\textbf{error}\xspace}%
  \newcommand{\PROGRAM}{\textbf{program}\xspace}%
  \newcommand{\PROCEDURE}{\textbf{procedure}\xspace}%
  \newcommand{\FUNCTION}{\textbf{function}\xspace}%
  \newcommand{\LET}{\textbf{let}\xspace}%
  \newcommand{\IF}{\textbf{if}\xspace}%
  \newcommand{\THEN}{\textbf{then}\xspace}%
  \newcommand{\ELSE}{\textbf{else}\xspace}%
  \newcommand{\WHILE}{\textbf{while}\xspace}%
  \newcommand{\FOR}{\textbf{for}\xspace}%
  \newcommand{\DO}{\textbf{do}\xspace}%
  \newcommand{\AND}{\textbf{and}\xspace}%
  \newcommand{\BREAK}{\textbf{break}\xspace}%
  \newcommand{\CONTINUE}{\textbf{continue}\xspace}%
  \newcommand{\OR}{\textbf{or}\xspace}%
  \newcommand{\NOT}{\textbf{not}\xspace}%
  \newcommand{\END}{\textbf{end}\xspace}%
  \newcommand{\RETURN}{\textbf{return}\xspace}%
}{%
}

\newenvironment{algorithm*}%
{%
\begin{BasicCommands@algorithm}%
\list{}{\itemindent 0em%
        \listparindent\itemindent
        \rightmargin  \leftmargin}%
\item\relax
}{%
\endlist
\end{BasicCommands@algorithm}%
}

\newenvironment{algorithm}%
{%
  \newcommand{\ResetLineCounter}{%
    \setcounter{LineCounter@algorithm}{0}%
  }%
  % \LN increases the line counter and produces the line number.
  % This command should be used only at the begining of the line.
  \newcommand{\LN}{%
    \makebox[0pt][l]{%
      \makebox[0pt][l]{%
        \addtocounter{LineCounter@algorithm}{1}%
      }%
      \makebox[10.75pt][r]{
        \fontsize{7}{10}%
        \selectfont%
        \arabic{LineCounter@algorithm}:%
      }%
    }%
    \TAB%
  }%
  % Tabulation mark
  \begin{BasicCommands@algorithm}%
  \begin{float@algorithm}%
    \ResetLineCounter%
}%
{%
  \end{float@algorithm}%
  \end{BasicCommands@algorithm}%
}


\newcommand{\new}[1]{{\color{black}#1}}




==> moreexp.tex <==
Table~\ref{fig:exp2} summarizes our performance when sampling updates based on their relative size compared to that of the underlying base instance (and not, 
as in Table~\ref{fig:exp1}, based on the relative percentage of symbols). Note that the gains are worse than the ones in Sec.~\ref{sec:eval}, even including
cases when maintenance is more costly than recomputation. Such instance-driven settings are indeed the worst-case scenario for our engine. The reason is that,
when dealing with large updates concerning a given symbol, the fine grained incrementality and stratified features of our engine
weight less that the very intense strain put on the join computation. 

\begin{table}[!ht]
\centering
\begin{tabular}{l|llll|llll} 
\multirow{2}{*}{$\rho$} & \multicolumn{3}{c}{WD}  & \multicolumn{3}{c}{SNB} \\ 
               & FVM & IVM & Diff  & Ratio Gain &  FVM & IVM & Diff  & Ratio Gain \\
 0.05         & 259.59  & 274.42   & -14.83 & -5.71\% FVM& 47.02  &      41.25  &  5.77 & 12.27\% FVM    \\
 0.1          & 267.72   &    260.68 & 7.04 & 2.62\% FVM & 45.31 &     40.92 &  4.39  & 9.68\% FVM   \\
 0.15         & 262.41   &   274.23 & -11.82 & -4.5\% FVM & 43.52 &  40.92     &  2.6 & 5.97\% FVM   \\
 0.2           &  200.77   &   219.27 & -18.5 & -9.21\% FVM &  39.3 &    38.95 &  0.35 & 0.89\% FVM    \\
 0.25          &  200.86    &  221.96 & -21.1 & -10.5\% FVM & 39.14 &   39.99  &  -0.85 & -2.17\% FVM
\end{tabular}
\vspace{2mm}
\caption{Average Workload Runtimes (ms) for Fized Instance Size $|\mathcal{G}_{LSN}| = |\mathcal{G}_{WD}| = 1K$ and
Instance-Driven Sampling with Varying Update Size ($\rho$) }
\label{fig:exp2}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

